API Pack: A Massive Multi-Programming Language Dataset for API Call Generation

We introduce API Pack, a massive multi-programming language dataset containing over one million instruction-API calls for improving the API call generation capabilities of large language models. Our evaluation highlights three key findings: First, fine-tuning on API Pack enables open-source models to outperform GPT-3.5 and GPT-4 in generating code for entirely new API calls. We show this by fine-tuning CodeLlama-13B on 20,000 Python instances from API Pack. Second, fine-tuning on a large dataset in one language, combined with smaller datasets from others, improves API generation accuracy across multiple languages. Third, we confirm the benefits of larger datasets for API generalization, as increasing fine-tuning data to one million instances enhances generalization to new APIs. To support further research, we open-source the API Pack dataset, trained model, and code at https://github.com/zguo0525/API-Pack.

==> sections/broader_impact.tex <==
% \section{Broader Impact Statement}
% \label{sec:broader_impact}

% This paper explores integrating API call and tool-based Large Language Models (LLMs) into code generation, with several pertinent broader impacts:

% \begin{itemize}

% \item \textbf{Enhanced Software Productivity:} The presented advancements promise significant software development acceleration by automating routine coding tasks. This could enable faster iterations, reduced costs, and potentially higher-quality products. However, reliance on auto-generated code risks reduced developer accountability and control.

% \item \textbf{Sociotechnical Considerations:} Although intelligent coding tools enhance productivity, concerns exist regarding job displacement and the need for continuous oversight to ensure accuracy. Further, enhanced access to code generation raises ethical questions around ownership, malicious use, and digital inequality.

% \item \textbf{Responsible Innovation:} Alongside promising productivity gains, the integration of advanced LLMs into software development workflows raises important challenges requiring proactive addressing by researchers and practitioners. A responsible innovation lens assessing and responding to potential harms remains vital.

% \end{itemize}

% This research aims to progress machine learning, but acknowledges associated societal impacts. Advancing coding-focused LLMs in an ethical, inclusive and responsible manner necessitates engaging with these multifaceted implications. This underscores the importance of considering both applications and consequences when embedding emerging technologies into real-world coding contexts.

% This research aims to progress machine learning, but acknowledges associated societal impacts. Advancing coding-focused LLMs in an ethical, inclusive and responsible manner necessitates engaging with these multifaceted implications. This underscores the importance of considering both applications and consequences when embedding emerging technologies into real-world coding contexts.

% \section{Broader Impact Statement}
% \label{sec:broader_impact}
% Our research has a broader impact on Software Productivity as it accelerates software development workflows by automating routine tasks. That said, the integration of advanced LLMs into software development workflows also raises negative sociotechnical concerns, such as job displacement. API Pack was designed to leaverage the creation of tools that increase software productivity by keeping humans in the loop, as it helps to 

% evelopers' continuous oversight to ensure accuracy)

% Therefore, a responsible innovation lens assessing and responding to potential harms remains vital.




==> sections/future_work.tex <==
\section{Future Work}
\label{sec:future_work}
% \textcolor{red}{
% \begin{itemize}
%     \item Dataset v2: API call classification to remove the need of API name in the instructions
%     \item Augmenting the dataset to include API calls with argument values
%     \item Augmenting the dataset to include Multi-API call scenarios
%     \item other experiments?
% \end{itemize}
% }
% \textcolor{red}{Overcoming these challenges is crucial for the development of more sophisticated and context-aware code generation models.}

Building upon these promising findings, we propose three future research directions:

\begin{itemize}
\itemsep0.01em
\item \textbf{Enriched API Classification.} Eliminating the explicit need of  API names in dataset instructions to allow intuitive context-based translation that better resembles natural coding workflows.

\item \textbf{Argument Augmentation.} Incorporating API calls with arguments for comprehensive, functional examples. This expanded scope enables models to generate detailed, actionable code that developers can test.

\item \textbf{Multi-Step API Scenarios.} Including multi-API call sequences to mirror real-world complexity and dependencies in advanced development settings.

% \item \textbf{Enhanced Architectures and Methods.} Exploring techniques like hierarchical modeling and prompt/example tuning to boost efficiency and task alignment for diverse coding settings.

\end{itemize}

% Advancing these areas aims not only to progress AI coding capabilities, but also address limitations in capturing the nuanced complexities of applied development environments. The ultimate objective is naturalistic models excelling in the intricacies of real-world coding across languages, tools, and interfaces. This necessitates co-design with practitioners focused on deployability beyond benchmarks. Ethical alignment also remains paramount as these systems integrate increasingly into creative software workflows.

==> sections/limitations.tex <==
\section{Limitations and Future Work}
\label{sec:limitations}

% The absence of license details in the OAS files is an issue that requires resolution, and thus, it has been prioritized in our ongoing work plan (Section 7). Though, resolution will take time. That said, we do have license information for the API Hubs (i.e., API-gurus - CC0-1.0 license), we will incorporate this information into our manuscript (Table 2).
% For data owners who wish to withdraw their information from our dataset, we have established a clear protocol. Please refer to the "Requesting Data Removal" section in our repository for detailed instructions (https://github.com/zguo0525/API-Pack).

\red{The first release of API Pack exhibits several limitations. One limitation is our evaluation methodology. We acknowledge that execution-based metrics like the pass rate or hallucination rate could provide a more robust evaluation. However, our focus on privacy protection and PII removal from the API database makes execution-based evaluation difficult with the current dataset structure. Additionally, API Pack was not designed for multi-API call scenarios, and the current instruction style requires specifying the API name, its application to complex software development scenarios may require additional work from end-users. Further, API Pack's coverage of programming languages is limited by the library used to generate code, meaning that a specific programming language of interest for end-users may not be supported. Lastly, while license information at the hub level is publicly available (i.e., API-gurus - CC0-1.0 license), only a few OAS files contain license information at the API level. Thus, API Pack might not be compliant with rigorous license policies sometimes required by proprietary software development efforts.} 

\red{We plan to address these limitations in future versions of the dataset. For evaluation, we will explore ways to enable execution-based evaluation while maintaining privacy, possibly through synthetic API endpoints or sanitized test environments. We also plan to integrate multi-API call scenarios and instructions that simply require a task description, further increase programming language diversity, and track down accurate license information for as much APIs included in API Pack as it is possible.}

% API Pack is not designed for multi-API call scenarios, so models fine-tuned with this dataset may struggle with tasks involving multiple, interdependent API calls. This limitation restricts API Pack's effectiveness in complex, real-world software development tasks that often require multi-API integrations. Future work should focus on creating datasets and models that can effectively handle multi-API call scenarios, enabling the generation of more sophisticated and practical code solutions.

% Our approach exhibits core limitations in areas of chained tool usage with interdependent APIs, support for interactive result refinement, sensitivity to precise input wording deciding API calls, sample inefficiency for certain tools yielding limited useful calls, accounting for varying computational costs across APIs, potential bias in machine learning predictions disadvantageous to subgroups, constraints processing extensive documentation without preprocessing, and reliance on external instruction-following model capabilities. Addressing these limitations presents opportunities to enhance functionality, applicability, efficiency, fairness and interpretability of self-supervised tool utilization. Our release of the extensive dataset fuels continued progress in this rapidly evolving field toward more robust, multifaceted large language model integration with real-world tools.

% \textcolor{red}{
% \begin{itemize}
%     \item Intent-detection requires API name in the instruction
%     \item Multi-API call scenarios
% \end{itemize}
% }

% While advancing the field of code generation with API call integration our research presents limitations:
% \begin{itemize}
%     \itemsep0.01em
%     %\item \textbf{API Pack instructions must include the API name to achieve correct intent-detection.} This limitation hinders the model's ability to intuitively interpret and respond incomplete queries.
%     % \item \textbf{Challenges with Multi-API Call Scenarios:} The model currently struggles with scenarios involving multiple, interdependent API calls. This restricts its effectiveness in complex, real-world software development tasks that commonly require such multi-API integrations.
%     \item \textbf{Challenges with Multi-API Call Scenarios.} As API Pack is not a multi-API call dataset, the models fine-tuned with this dataset will potentially struggle with scenarios involving multiple, interdependent API calls. This restricts API Pack effectiveness in complex, real-world software development tasks.
% \end{itemize}

% Overcoming these challenges is crucial for the development of more sophisticated and context-aware code generation models.
